Description of the Operational Mechanics of a Basel Regulated Banking System

This paper presents a description of the mechanical operations of banking as used in modern banking systems regulated under the Basel Accords, in order to provide support for a verifiable and complete description of the banking system suitable for computer simulation. Feedback is requested on the contents of this document, both with respect to the operations described here, and any known national, regional or local variations in their structure and practice.

==> loan_default.tex <==
Losses on loans, either whole or partial write-offs are treated as an expense for Banks,
and are initially deducted from income. There are though several stages to this process, and additional 
and potentially systemic complexities also occur if
the capital reserve becomes involved. In general, loan write-offs are a somewhat predictable occurrance
for banks, several payments have to be missed before a loan is treated as impaired, and banks
are required to make and continuously adjust loss provisions that match their anticipated losses.
Banks also have some freedom
on how impaired loans are treated, and may elect to write off all or some of the loan, or refinance it.
\par
If loan losses and other expenses significantly exceed income, then
the capital reserve is used to cover the write-off. With respect to the Basel Accord Tier 1 and Tier
2 capital lending provisions, the bank may be over capitalised, in which case there is a buffer
of capital that can be used for this purpose without any impact on its ability to lend with respect to
its risk weighted capital reserve multiplier. regulatory situation. However,
since banks must maintain a limit on their lending that is a multiple of their Tier 1 \& 2 reserve
funds, if losses are sufficient they can push the bank out of regulatory
compliance, since it will no longer meet its capital requirement. This last situation is rarely
recoverable without external intervention.
\par
The book keeping arrangements that are used to represent the first part of this process
use a contra-asset account for loan losses,
which is then subtracted from gross loans.\footnote{A contra-asset account is an asset account
which has a credit balance, normally asset accounts maintain a debit balance. The contra-asset
account is itself linked to an asset account, and the book value is the net value of the two accounts.
It is effectively a way of carrying an offsetting allowance forward for loss provisions
or depreciations, linked to specific ledgers for tracking purposes.}
In the example below, we will begin with showing the creation of a loan loss account from income
received, and then assume that its contents are sufficient to cover losses from the loan writedown of
50 for Bank A.
\begin{table}[ht]
\centering
\begin{tabular}{lll}
\multicolumn{2}{l}{Operations} \\
\cline{1-2}
1) & debit interest account         & credit loss provisions account \\
2) & credit loan amount             & debit loss provisions account \\
\end{tabular}
\label{tab:loandefault}
\end{table}
The significance of the contra-asset designation of the loss provisions account becomes
clearer when the transfer from the interest income account is examined. The funds are
credited to the loss provisions account, but as it is a contra-asset account they act
to reduce the total asset balance.
\par
When the bank then writes off part of its loan book (50 in the example shown in Table \ref{tab:writeoff3},
the loss provision account is reduced by the amount of the writeoff, as is the loan book. Strictly,
the loss provision account is debited, reducing its balance, and the loan account is credited,
also reducing its balance, since it as an Asset account. The net balance of the Assets is unchanged
as a result, since the loss provision account has already accounted for the write off.
\par
As a result, the effect of the writeoff on the balance sheet usually precedes the actual writeoff,
which is of some significance when analysing a bank's position from its balance sheet. It is
worth noting, that as long as the loss can be covered from income, then the overall state
of the balance sheet (with respect to the reduction in assets caused by the writeoff) can be
restored by new lending. Nor are there any accompanying money supply considerations, since the
money removed from the system by the loan writeoff is replaced by the new loan. Some degree of
loan losses can consequently be absorbed by the system with no systemic repercussions for the
money supply. There may be implications for the larger economic debt supply, depending on the
subsequent treatment of the loan, which although removed from the bank's balance sheet,
may be sold on for collection. Local practices surrounding the handling of bankruptcy and recourse
and non-recourse lending will play a part there.
\input{writeoff1.tex}
\input{writeoff2.tex}
\input{writeoff3.tex}


